Network-Aware 5G Edge Computing for Object Detection: Augmenting Wearables to "See" More, Farther and Faster

Advanced wearable devices are increasingly incorporating high-resolution multi-camera systems. As state-of-the-art neural networks for processing the resulting image data are computationally demanding, there has been growing interest in leveraging fifth generation (5G) wireless connectivity and mobile edge computing for offloading this processing to the cloud. To assess this possibility, this paper presents a detailed simulation and evaluation of 5G wireless offloading for object detection within a powerful, new smart wearable called VIS4ION, for the Blind-and-Visually Impaired (BVI). The current VIS4ION system is an instrumented book-bag with high-resolution cameras, vision processing and haptic and audio feedback. The paper considers uploading the camera data to a mobile edge cloud to perform real-time object detection and transmitting the detection results back to the wearable. To determine the video requirements, the paper evaluates the impact of video bit rate and resolution on object detection accuracy and range. A new street scene dataset with labeled objects relevant to BVI navigation is leveraged for analysis. The vision evaluation is combined with a detailed full-stack wireless network simulation to determine the distribution of throughputs and delays with real navigation paths and ray-tracing from new high-resolution 3D models in an urban environment. For comparison, the wireless simulation considers both a standard 4G-Long Term Evolution (LTE) carrier and high-rate 5G millimeter-wave (mmWave) carrier. The work thus provides a thorough and realistic assessment of edge computing with mmWave connectivity in an application with both high bandwidth and low latency requirements.

==> abstract.tex <==
%% Abstract
Advanced wearable devices are increasingly 
incorporating  high-resolution multi-camera systems.
As state-of-the-art neural networks for 
processing the resulting image data are 
computationally demanding, there
has been growing interest in leveraging
\gls{5g} wireless connectivity and
mobile edge computing for offloading
this processing to the cloud.  To assess this possibility, 
this paper presents a detailed simulation 
and evaluation of \gls{5g} wireless offloading
for object detection within a powerful, new 
smart wearable called \VISION, for the Blind-and-Visually Impaired (BVI).
The current \VISION system is an instrumented
book-bag with high-resolution
cameras, vision processing and haptic and audio
feedback. The paper considers uploading the camera 
data to a mobile edge 
cloud to perform real-time object detection and transmitting the detection results  
back to the wearable.  
To determine the video requirements, the paper evaluates
the impact of video bit rate and resolution on object detection
accuracy and range. A new 
street scene dataset with labeled objects relevant to BVI navigation is leveraged for analysis. The vision evaluation
is combined with a detailed full-stack
wireless network simulation 
to determine the distribution of throughputs and delays 
with real navigation paths and ray-tracing
from new high-resolution 
3D models in an urban environment. 
For comparison, the wireless simulation considers
both a standard 4G-\gls{lte} carrier and 
high-rate \gls{5g} \gls{mmw} carrier.
The work thus provides a thorough
and realistic assessment of edge computing
with \gls{mmw} connectivity in an application with 
both high bandwidth and low latency requirements.






==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yuan}}]{Zhongzheng (Jacky) Yuan} received the B.S. and M.S. in electrical engineering from the New York University Tandon School of Engineering, Brooklyn, NY, USA, in 2019 and 2020, respectively. He had held internship positions in Media Lab at Tencent America, and Incubation Lab at Dolby Laboratories.

He is currently a Ph.D. candidate in electrical engineering at New York University, under the supervision of Prof. Yao Wang. His research interests include image/video compression, computer vision, and deep learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/azzino}}]{Tommy Azzino}  received the B.Sc. and M.Sc. in information engineering and telecommunications engineering, respectively, from the University of Padova, Italy, in 2016 and 2019. He is currently pursuing the Ph.D. degree in electrical and computer engineering with New York University Tandon School of Engineering, Brooklyn, NY, USA, under the supervision of Prof. S. Rangan. He held visiting research positions with the National Institute of Standards and Technology (NIST), Department of Commerce, Gaithersburg, MD, USA, in 2018, Nokia Bell Labs France, Paris, France, in 2019.

He took part to the 2018 edition of the Seeds for the Future Project promoted by Huawei Technologies in Shenzhen, PRC, in 2018. His research interests include 5G mobile cloud/edge computing, 5G network simulation and prototyping, MAC and network-layer resource allocation, wireless communications, and machine learning  for wireless communications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/hao}}]{Yu Hao} received his B.Eng degree in Computer Science and Technology from Beijing University of Technology, Beijing, China in 2019. He received an M.S degree in Computer Science from New York University, New York, USA in 2021. He is currently pursuing the Ph.D. degree in Computer Science at New York University. His research interests include Computer Vision, Computer Graphics, and Deep Learning. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/lyu}}]{Yixuan Lyu} was born In Beijing, China in 1996. He received a B.E. degree in automation from Nanjing University of Science and Technology in 2019 and now pursuing a master’s degree in New York University majoring in Computer Engineering. His research interests include video/image compression methods, computer vision, and deep neural networks.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/pei}}]{Haoyang Pei} was born In Yuncheng, Shanxi, China in 1995. He received a B.E. degree in electrical engineering and its automation from North China Electric Power University in 2017 and now pursuing a master's degree in New York University majoring in Computer Engineering. His research interests include video/image compression, computer vision, and deep learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/boldini}}]{Alain Boldini} received B.Sc. degree in Aerospace Engineering and M.Sc. degree in Aeronautical Engineering from Politecnico di Milano, Milan, Italy, in 2015 and 2017, respectively, and M.Sc. in Aerospace Engineering from Politecnico di Torino, Turin, Italy, in 2018.

He is currently a PhD candidate in Mechanical Engineering at the New York University Tandon School of Engineering. He is involved in research in smart advanced materials, assistive technologies, and dynamical systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/mezzavilla}}]{Marco Mezzavilla} received the B.A.Sc., the M.Sc., and the Ph.D. at the University of Padua, Italy, all in Electrical Engineering. He held visiting research positions at the NEC Network Laboratories in Heidelberg (Germany, 2009), at the Telematics Department at Polytechnic University of Catalonia (UPC) in Barcelona (Spain, 2010), and at Qualcomm Research in San Diego (USA, 2012).

He joined New York University (NYU) Tandon School of Engineering in 2014, where he is currently a Research Faculty and leads multiple mmWave-related research projects, mainly focusing on 5G and beyond PHY/MAC design. He is serving as reviewer for many IEEE and ACM conferences, journals, and magazines. His research interests include design and validation of communication protocols and applications for 5G and beyond broadband wireless technologies, millimeter-wave communications, multimedia traffic optimization, radio resource management, spectrum sharing, convex optimization, cognitive networks, and novel network paradigms. He is a Senior Member of the IEEE. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/beheshti}}]{Mahya Beheshti} received her M.D. degree from Gulf Medical University, School of Medicine, Ajman, UAE.

She is a Physician-scientist at NYU Langone Medical Center’s Rusk Rehabilitation. She is also pursuing the Ph.D. degree in Mechanical and Aerospace Engineering Department, NYU Tandon School of Engineering. She is the author of 3 book chapters, more than 17 peer-reviewed articles and 13 poster presentations. She has also given multiple talks. Her research interests lie within the realm of neurorehabilitation, human-machine interface, specifically EEG-based pattern recognition and wearable technologies.

Dr. Beheshti was a recipient of Distinguished Alumni Award of Healthcare Academia from Gulf Medical University and was chosen as Intern of the Year during her medical training. She is a member of American Society of Neuroradiology (ASNR), American Medical Association (AMA), National Multiple Sclerosis Society, and Association of Academic Physiatry (AAP). She is IEEE student member (IEEE RAS, IEEE EMBS, and IEEE WIE).
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/porfiri}}]{Maurizio Porfiri} (Fellow, IEEE) received the M.Sc. and Ph.D. degrees in engineering mechanics from Virginia Tech, Blacksburg, VA, USA, in 2000 and 2006, respectively, and the “Laurea” (Hons.) degree in electrical engineering and the Ph.D. degree in theoretical and applied mechanics from the Sapienza University of Rome, Rome, Italy, and the University of Toulon, Toulon, France (under a dual-degree program between Italy and France), in 2001 and 2005, respectively.

He is currently an Institute Professor with the New York University Tandon School of Engineering, Brooklyn, NY, USA, having appointments with the Center for Urban Science and Progress, Department of Mechanical and Aerospace Engineering, Department of Biomedical Engineering, and Department of Civil and Urban Engineering. He is the Director of the Dynamical Systems Laboratory. He is involved in conducting and supervising research on dynamical systems theory and applications. He has authored more than 350 journal publications. He has been included in the “Brilliant 10” list of Popular Science in 2010. His research featured in major media outlets, including CNN, NPR, Scientific American, and Discovery Channel.

Dr. Porfiri is the recipient of the National Science Foundation CAREER Award, the Outstanding Young Alumnus Award by the College of Engineering, Virginia Tech, the American Society of Mechanical Engineers (ASME) Gary Anderson Early Achievement Award, the ASME DSCD Young Investigator Award, and the ASME C.D. Mote, Jr. Early Career Award. His other significant recognitions include invitations to the Frontiers of Engineering Symposium and the Japan–America Frontiers of Engineering Symposium organized by the National Academy of Engineering He has served on the Editorial Board of the ASME Journal of Dynamics Systems, Measurements and Control, the ASME Journal of Vibrations and Acoustics, Flow, the IEEE CONTROL SYSTEMS LETTERS, the IEEE TRANSACTIONS ON CIRCUITS AND SYSTEMS I: REGULAR PAPERS, and Mechatronics. He is a Fellow of the ASME.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/hudson}}]{Todd E. Hudson} is an Assistant Professor of Rehabilitation Medicine at New York University’s Grossman School of Medicine, holding cross-appointments in Neurology, and also in the Department of Biomedical Engineering at the New York University Tandon School of Engineering.

Prof. Hudson is a Computational Neuroscientist whose research focuses on modeling sensory and motor systems, particularly with regard to eye and arm movements in healthy and disease states, movement planning, and spatial orientation. He received his PhD from Columbia University, and has authored over 50 peer reviewed articles, as well as the textbook ‘Bayesian Data Analysis for the Behavioral and Neural Sciences’ from Cambridge University Press.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/seiple}}]{William Seiple} received the B.S. and M.S. degrees in psychology from the Albright College, Reading, PA and the University of North Carolina, Greensboro, NC and the Ph.D. degree in zoology from the University of Illinois, Urbana, IL.

He is the Chief Research Officer at Lighthouse Guild, Research Professor of Ophthalmology at New York University School of Medicine,  and Adjunct Faculty at the Institut de la Vision, Paris. He is the author of two books chapters, and more than 150 peer-reviewed articles.

His research interests include development and assessment of functional interventions for people with vision loss, rehabilitation training, and visual electrophysiology and psychophysics of vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/fang}}]{Yi Fang} received the BS and MS degrees in biomedical engineering from Xi’an Jiaotong University, Xi’an, China, in 2003 and 2006, respectively, and the PhD degree in mechanical engineering from Purdue University, West Lafayette, Indiana, in 2011.

He is currently an assistant professor with the Department of Electrical and Computer Engineering, New York University Abu Dhabi, Abu Dhabi, United Arab Emirates. His research interests include three-dimensional computer vision and pattern recognition, large-scale visual computing, deep visual computing, deep cross-domain and cross modality multimedia analysis, and computational structural biology.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/rangan}}]{Sundeep Rangan}  received the B.A.Sc. at the University of Waterloo, Canada and the M.Sc. and Ph.D. at the University of California, Berkeley, all in Electrical Engineering. He has held postdoctoral appointments at the University of Michigan, Ann Arbor and Bell Labs.  In 2000, he co-founded (with four others) Flarion Technologies, a spin-off of Bell Labs, that developed Flash OFDM, the first cellular OFDM data system and pre-cursor to 4G cellular systems including LTE and WiMAX. In 2006, Flarion was acquired by Qualcomm Technologies.  Dr. Rangan was a Director of Engineering at Qualcomm involved in OFDM infrastructure products. He joined NYU Tandon (formerly NYU Polytechnic) in 2010 where he is currently a Professor of Electrical and Computer Engineering.  He is a Fellow of the IEEE and the Associate Director of NYU WIRELESS, an industry-academic research center on next-generation wireless systems.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/wang}}]{Yao Wang} is a Professor at New York University Tandon School of Engineering (formerly Polytechnic University, Brooklyn, NY), with joint appointment in Departments of Electrical and Computer Engineering and Biomedical Engineering. She is also Associate Dean for Faculty Affairs for NYU Tandon since June 2019. Her research areas include video coding and streaming, multimedia signal processing, computer vision, and medical imaging. 

She is the leading author of a textbook titled Video Processing and Communications, and has published over 250 papers in journals and conference proceedings. She received New York City Mayor's Award for Excellence in Science and Technology in the Young Investigator Category in year 2000. She was elected Fellow of the IEEE in 2004 for contributions to video processing and communications. She received the IEEE Communications Society Leonard G. Abraham Prize Paper Award in the Field of Communications Systems in 2004, and the IEEE Communications Society Multimedia Communication Technical Committee Best Paper Award in 2011. She was a keynote speaker at the 2010 International Packet Video Workshop, INFOCOM Workshop on Contemporary Video in 2014,  the 2018 Picture Coding Symposium, and the 2020 ACM Multimedia Systems Conference (MMSys’20). She received the NYU Tandon Distinguished Teacher Award in 2016.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/rizzo}}]{John-Ross (JR) Rizzo} was born in Wayne, NJ, USA. He received his medical degree from New York Medical College, Alpha Omega Alpha Honors, on academic scholarship.

He is currently a physician-scientist at NYU Langone Medical Center’s Rusk Rehabilitation, where he serves as vice chair of Innovation and Equity for Physical Medicine and Rehabilitation with cross-appointments in the Department of Neurology and the Departments of Biomedical \& Mechanical and Aerospace Engineering at NYU-Tandon School of Engineering. He is also the Associate Director of Healthcare for the NYU Wireless Laboratory in the Department of Electrical and Computer Engineering at NYU-Tandon. He leads the Visuomotor Integration Laboratory (VMIL) and the REACTIV Laboratory (Rehabilitation Engineering Alliance and Center Transforming Low Vision), where his team focuses on assistive technology for the visually impaired and benefits from his own personal experiences with vision loss.  He is the author of 10 book chapters, more than 80 peer-reviewed articles and many poster presentations. His research interests lie within the realm of neurorehabilitation, assistive technologies, and health equity. 

Dr. Rizzo was awarded the prestigious Crain’s 40 under 40 award in New York Business for his medical devices, including his wearable technology. He has also been featured in several lay articles and also featured in videos and press releases. In 2018, he was a highlighted speaker in NYU’s TEDx “Re-Vision” Series. He is a member of American Medical Association, American College of Physicians, American Academy of PM\&R (AAPM\&R), Association of Academic Physiatry (AAP), and American Heart Association.
\end{IEEEbiography}
